Time complexity of concurrent programs

We study the problem of automatically computing the time complexity of concurrent object-oriented programs. To determine this complexity we use intermediate abstract descriptions that record relevant information for the time analysis (cost of statements, creations of objects, and concurrent operations), called behavioural types. Then, we define a translation function that takes behavioural types and makes the parallelism explicit into so-called cost equations, which are fed to an automatic off-the-shelf solver for obtaining the time complexity.

==> runtime-typing.tex <==
In order to prove the correctness of our system, we need to be able
 to show that
 \begin{enumerate}
 \item\label{item1} the behavioural type is preserved by the reduction, and
  \item\label{item2} the time cost computed by our system is an upper bound of the actual cost of the computation.
  \end{enumerate}

  For proving~\ref{item1} we need first to extend the type system of Section~\ref{sec:typesystem} to extract behavioural types for runtime configurations.
  The extended runtime type syntax include also the following category:

  {\footnotesize
  \begin{syntax}
    \simpleentry 
    \concntc [] \quad 
    \cntb \bnfor \cinvoc{f}{c}{\cntb } \bnfor \concntc\parallel\concntc
    \qquad \qquad [runtime behavioural type]
  \end{syntax}
}

Behavioral type $\cntb$ is as before, while $\cinvoc{f}{c}{\cntb }$ expresses the behavior of
an asynchronous method referenced by future $f$ and running in cog $c$.

The runtime environment $\Delta$ is defined as $\Gamma$ extended with
the mapping of objects to values.

The behavioral type preservation is now expressed by a subject
reduction theorem, where the behavioral type of the reduced
configuration is proved to be in a \emph{later-stage} relation,  defined in Figure~\ref{fig:sr:lr}, with
the type of the reduct configuration.



\begin{theorem}[Subject Reduction]\label{th_subjred}
Let $\Delta\typep \nt{cn}\typed \concntc$ and $\nt{cn}\rightarrow \nt{cn}'$.
Then there exist $\Delta'$,  $\concntc'$, and an injective renaming of 
cog names $\imath$ such that 
\begin{itemize}
\item[--] $\Delta' \vdash \nt{cn}'\typed \concntc'$ and
\item[--] $\imath(\concntc)\cls\concntc'$.
\end{itemize}
\end{theorem}


% {\footnotesize
%   \begin{syntax}
%  \simpleentry 
%     \frt [] \quad \unit \bnfor se \bnfor \cogty{c}{\nt{se}}
%     [basic value]   
%     \\
%     \simpleentry 
%     \frx [] \quad f \bnfor \frt
%     [extended value]
%     \\
%     \simpleentry
%     \cntcel [] \quad 
%     e \bnfor \nucogty{c}{\nt{se}} \bnfor
%     \mty{\m}{\vect{\frt}} \rightarrow \frt \bnfor
%     \newel{f}{\mty{\m}{\vect{\frt}} \rightarrow \frt} \bnfor 
%     \rmel{f} \qquad 
%     [atom]
%     \\
%     \simpleentry 
%     \cntb [] \quad 
%     \cntcel \triangleright \Gamma \bnfor \cntcel
%     \fatsemi \cntb \bnfor (\nt{se}) \{\cntb\} \bnfor \cntb + \cntb 
%     \qquad \qquad [behavioural type]
%     \\
%     \simpleentry 
%     \concntc [] \quad 
%     \cntb \bnfor \cinvoc{f}{c}{ \cntb } \bnfor \concntc\parallel\concntc
%     \qquad \qquad [runtime behavioural type]
%   \end{syntax}
% }

The typing rule for runtime configuration are reported in Figure~\ref{fig:rntyp}.

\begin{figure*}[t]
 \begin{rules}
\entry[{\scriptsize (TR-Future)}]{\Delta(f)=\fty{\m}{\frt_r}\\
\nt{val}\neq\bot\Rightarrow\Delta \vdash \nt{val}: \frt_r}
{\Delta\vdash \textit{fut}(f,\nt{val})\typed\pinull}
\and
\entry[{\scriptsize
  (TR-Invoc)}]{\Delta(f)=\fty{\m}{\frt_r}\\
  \typepe{\Delta}{\mty{\m}{\cogty{c}{se},\vect{\frt}}}{\frt_r} \\\typepe{\Delta}{\many{v}}{\many{\frt}} \\  \Delta(o)=\cogty{c}{se}}
  {\Delta\vdash \textit{invoc}(o,f,m,\many{v})\typed\cinvoc{f}{c}{ \mtyR{\m}{\cogty{c}{se},\bar{\frt}}{\frt_r} }}
  \and
  \entry[{\scriptsize (TR-Cog)}]{
     \typepe{\Delta}{c}{\const}}
  {\Delta\vdash \textit{cog}(c,\nt{act},\const)\typed\btnull}
\and
\entry[{\scriptsize (TR-Object)}]{\Delta(o)=\cogty{c}{\nt{se}}\\
    \Delta \vdash^{c}_{o} p:\concntc\\
    \forall i\in \{1..n\}.~\Delta \vdash^{c}_{o} p_i\typed\concntc_i}
  {\Delta\vdash ob(o, c, p, p_1\cdots
    p_n):\concntc\parallel\concntc_1\parallel\cdots\parallel \concntc_n}
\and
\entry[{\scriptsize (TR-Process)}]{
	\Delta\vdash^{c}_{o} \many{\nt{val} : \frx} 
	 \\
	 \Delta(f)=\fty{\m}{\frt_r}
	\\\\
	\Delta[\text{destiny} \mapsto \frt_r, \many{x\mapsto\frx}]\vdash^{c}_{o} \nt{s}\typed\cntb}
  {\Delta\vdash^{c}_{o} \{\text{destiny} \mapsto f, \dl\mapsto \const,\many{\ x \mapsto \nt{val}} \; |\,\nt{s}\}: \cinvoc{f}{c}{\cntb}}
\and
\simpleentry[{\scriptsize (TR-Idle)}]{\Delta\vdash^{c}_{o} \key{idle}\typed\btnull}
\and
\entry[{\scriptsize(TR-Parallel)}]{\Delta\vdash cn_1\typed\concntc_1\\\Delta\vdash cn_2\typed\concntc_2}{\Delta\vdash cn_1\ cn_2\typed\concntc_1\parallel\concntc_2}
\end{rules}
\caption{The typing rules for runtime configurations.}
\label{fig:rntyp}
\end{figure*}

The runtime typing rules for expressions are reported in
Figure~\ref{fig:runtypesystem}. The ones for statements are reported
in Figure~\ref{fig:runtypesystem-stm}
%
\begin{figure}[t]
{\footnotesize
\[
\begin{array}{@{\hspace*{-1cm}}c}
    \mathrule{RT-Obj}{
      o\in\dom(\Delta)
    }{
      \typepe{\Delta}{o}{\Delta(o)}
    }
    \quad
    \mathrule{RT-Fut}{
      f\in\dom(\Delta)
    }{
      \typepe{\Delta}{f}{\Delta(f)}
  }
  \quad
    \mathrule{RT-Var}{
      x\in\dom(\Delta)
    }{
      \typepe{\Delta}{x}{\Delta(x)}
    }
    \qquad
    \mathax{RT-Se}{
      \typepe{\Delta}{\nt{se}}{\nt{se}}
    }
    \qquad
    \mathax{RT-Nse}{
      \typepe{\Delta}{\nt{nse}}{\unit}
    }
  \\
  \\
    \mathrule{RT-Method}{
      \begin{array}{c}
      \Delta(\m) = (\vect{\frt}) \rightarrow \frt' 
      \\
      \fv(\frt') \setminus \fv(\vect{\frt}) \neq \emptyset
      \quad \text{implies} \quad \sigma(\frt') \fresh
      \end{array}
    }{
      \typepe{\Delta}{
        \mty{\m}{\sigma(\vect{\frt})}
      }{\sigma(\frt')} 
    }
    \qquad
    \mathrule{RT-New}{
      \typepe{\Delta}{e}{\nt{se}}
      \quad
      c' \fresh
    }{
      \typeeeR{\Delta}{c}{o}{\new \Class\ \key{with}\ e}{\cogty{c'}{\nt{se}}}{\nucogty{c'}{\nt{se}}\triangleright 
        \Delta[c'\mapsto \nt{se}]} 
    }
    \\\\
    \mathax{RT-New-Local}{
      \typeeeR{\Delta}{c}{o}{\newloc \Class}{\cogty{c}{\nt{se}}}{\btnull\triangleright 
        \Delta} 
    }
    \qquad
    \mathrule{RT-Invoke}{
    \begin{array}{c}
      \typepe{\Delta}{e}{\cogty{c'}{\nt{se}}}
      \quad
      (c' \in \dom(\Delta) \quad \mbox{or} \quad c=c')
      \\
      \typepe{\Delta}{\vect{e}}{\vect{\frt}}
      \quad
      \typepe{\Delta}{\mty{\m}{\cogty{c'}{\nt{se}},\vect{\frt}}}{\frt'}
      \quad
      f \fresh
      \end{array}
    }{
      \typeeeR{\Delta}{c}{o}{e \async \name m(\vect e)}{f}{\newel{f}{\mty{\m}{\cogty{c'}{\nt{se}},\vect{\frt}}\rightarrow \frt'} \triangleright 
        \Delta[f \mapsto \frt']} 
    }
      \\\\
    \mathrule{RT-Get}{
      \typepe{\Delta}{e}{f}
      \quad
      \Delta(f) = {\frt_r}    }{
      \typeeeR{\Delta}{c}{o}{\eget e}{\frt_r}{\rmel{f}\triangleright 
        \Delta[f\mapsto \rmel{\frt_r}]} 
    }
    \qquad
    \mathrule{RT-Get-Top}{
      \typepe{\Delta}{e}{f}
      \quad
      \Delta(f) = {\rmel{\frt_r}}
    }{
      \typeeeR{\Delta}{c}{o}{\eget e}{\frt_r}{\btnull \triangleright 
        \Delta} 
    }
    \\\\
    \mathrule{RT-Invoke-Sync}{
    	\begin{array}{c}
      \typepe{\Delta}{e}{\cogty{c}{\nt{se}}}
      %\quad
      %\Delta(o)=\cogty{c}{\nt{se}}
      \\
      \typepe{\Delta}{\vect{e}}{\vect{\frt}}
      \quad
      \typepe{\Delta}{\mty{\m}{\cogty{c}{\nt{se}},\vect \frt}}{\frt'}
      \end{array}
    }{
      \typeeeR{\Delta}{c}{o}{e.\name m(\vect e)}{\frt'}{\mty{\m}{\cogty{c}{\nt{se}},\vect{\frt}}\rightarrow \frt'\triangleright 
        \Delta} 
    }
  \end{array}
  \]}
  \caption{Runtime typing rules for expressions}
  \label{fig:runtypesystem}
\end{figure}
\begin{figure}[t]
{\footnotesize
\[
  \begin{array}{c}
    \mathrule{RT-Assign}{
      \typeeeR{\Delta}{c}{o}{\nt{rhs}}{\frx}{\cntcel \triangleright \Delta'}
    }{
      \typestR{\Delta}{c}{o}{x = \nt{rhs}}{\cntcel \triangleright 
        \Delta'[x\mapsto \frx]} 
    }
    \qquad
    \mathrule{RT-Job}{
      \typepe{\Delta}{e}{\nt{se}}  
      \quad
      \typepe{\Delta}{o}{\cogty{c}{\nt{se}'}} 
    }{
      \typestR{\Delta}{c}{o}{\job{e}}{\nt{se}/\nt{se}' \triangleright 
        \Delta} 
    }
    \\\\
    \mathrule{RT-Return}{
      \typepe{\Delta}{e}{\frt}
      \quad
      \typepe{\Delta}{\destiny}{\frt}
    }{
      \typestR{\Delta}{c}{o}{\ereturn e}{\btnull \triangleright 
        \Delta} 
    }
    \qquad
    \mathrule{RT-Seq}{
    	\begin{array}{c}
      \typestR{\Delta}{c}{o}{s}{{\cal C}[\cntcel_1 \triangleright
        \Delta_1] \cdots [\cntcel_n \triangleright \Delta_n]} 
      \\
      \typestR{\Delta_i}{c}{o}{s'}{\cntb_i'}
      \end{array}
    }{
      \typestR{\Delta}{c}{o}{s\semi s'}{{\cal C}[\cntcel_1 \fatsemi
        \cntb_1'] \cdots [\cntcel_n \fatsemi \cntb_n'] } 
    }
    \\\\
    \mathrule{RT-If-Nse}{
      \typepe{\Delta}{e}{\unit}
      \quad
      \typestR{\Delta}{c}{o}{s}{\cntb}
      \quad
      \typestR{\Delta}{c}{o}{s'}{\cntb'}
    }{
      \typestR{\Delta}{c}{o}{\eif{e}{s}{s'}}{\cntb + \cntb'} 
    }
    \qquad
    \mathrule{RT-If-Se}{
      \typepe{\Delta}{e}{\nt{se}}
      \quad
      \typestR{\Delta}{c}{o}{s}{\cntb}
      \quad
      \typestR{\Delta}{c}{o}{s'}{\cntb'}
    }{
      \typestR{\Delta}{c}{o}{\eif{e}{s}{s'}}{(\nt{se}) \{\cntb\} +
        (\neg\nt{se}) \{\cntb'\}}  
    }
  \end{array}
  \]}
  \caption{Runtime typing rules for statements}
  \label{fig:runtypesystem-stm}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

